Using Household Grants to Benchmark the Cost Effectiveness of a USAID Workforce Readiness Program

We use a randomized experiment to compare a workforce training program to cash transfers in Rwanda. Conducted in a sample of poor and underemployed youth, this study measures the impact of the training program not only relative to a control group but relative to the counterfactual of simply disbursing the cost of the program directly to beneficiaries. While the training program was successful in improving a number of core outcomes (productive hours, assets, savings, and subjective well-being), cost-equivalent cash transfers move all these outcomes as well as consumption, income, and wealth. In the head-to-head costing comparison cash proves superior across a number of economic outcomes, while training outperforms cash only in the production of business knowledge. We find little evidence of complementarity between human and physical capital interventions, and no signs of heterogeneity or spillover effects.

==> tables/employment_breakdown_A.tex <==
\begin{tabular}{l *{6}{S} ScSS}
\toprule
 & & \multicolumn{4}{c}{GiveDirectly} & & \multicolumn{1}{c}{\raisebox{-1ex}[0pt]{Control}} \\ 
\cmidrule(lr){3-6}
\multicolumn{1}{c}{\text{ }} & \multicolumn{1}{c}{\text{HD}} & \multicolumn{1}{c}{\text{Lower}} & \multicolumn{1}{c}{\text{Middle}} & \multicolumn{1}{c}{\text{Upper}} & \multicolumn{1}{c}{\text{Large}} & \multicolumn{1}{c}{\text{Combined}} & \multicolumn{1}{c}{\text{Mean}} & \multicolumn{1}{c}{\text{Obs.}} & \multicolumn{1}{c}{\text{$ R^2$}} & \multicolumn{1}{c}{\text{$ p$-value}}\\
\midrule
\multicolumn{11}{l}{\emph{Panel A. Employment composition}}  \\ 
\addlinespace[1ex] \multirow[t]{ 3 }{0.2\textwidth}{Non-agricultural microenterprise }  &      0.05 &      0.09\ensuremath{^{*}} &      0.08\ensuremath{^{*}} &      0.14\ensuremath{^{**}} &      0.17\ensuremath{^{***}} &      0.12\ensuremath{^{**}} &      0.22 &      1770 &      0.12 &      0.00 \\ 
 & (0.03)  & (0.04)  & (0.04)  & (0.05)  & (0.04)  & (0.04)  \\  & [    0.11]  & [    0.06]  & [    0.08]  & [    0.02]  & [    0.00]  & [    0.02]  \\ \addlinespace[1ex] 
\multirow[t]{ 3 }{0.2\textwidth}{Other microenterprise or self-employment }  &      0.04\ensuremath{^{*}} &      0.04 &      0.11\ensuremath{^{**}} &      0.07\ensuremath{^{*}} &      0.05\ensuremath{^{*}} &      0.04 &      0.07 &      1770 &      0.09 &      0.02 \\ 
 & (0.02)  & (0.03)  & (0.03)  & (0.03)  & (0.03)  & (0.03)  \\  & [    0.06]  & [    0.11]  & [    0.02]  & [    0.06]  & [    0.09]  & [    0.11]  \\ \addlinespace[1ex] 
\multirow[t]{ 3 }{0.2\textwidth}{Agricultural processing or trading }  &      0.01 &      0.13\ensuremath{^{**}} &      0.01 &      0.07\ensuremath{^{*}} &      0.06 &      0.02 &      0.17 &      1770 &      0.08 &      0.05 \\ 
 & (0.03)  & (0.04)  & (0.04)  & (0.04)  & (0.04)  & (0.04)  \\  & [    0.24]  & [    0.02]  & [    0.24]  & [    0.08]  & [    0.11]  & [    0.24]  \\ \addlinespace[1ex] 
\multirow[t]{ 3 }{0.2\textwidth}{Agricultural wage labor }  &     -0.02 &     -0.08\ensuremath{^{**}} &     -0.07\ensuremath{^{*}} &     -0.08\ensuremath{^{**}} &     -0.11\ensuremath{^{**}} &     -0.09\ensuremath{^{**}} &      0.22 &      1770 &      0.15 &      0.00 \\ 
 & (0.03)  & (0.03)  & (0.03)  & (0.03)  & (0.03)  & (0.03)  \\  & [    0.24]  & [    0.03]  & [    0.06]  & [    0.03]  & [    0.02]  & [    0.03]  \\ \addlinespace[1ex] 
\multirow[t]{ 3 }{0.2\textwidth}{Non-agricultural wage labor }  &      0.06\ensuremath{^{*}} &     -0.04 &      0.01 &     -0.06 &     -0.07\ensuremath{^{*}} &      0.01 &      0.30 &      1770 &      0.20 &      0.00 \\ 
 & (0.03)  & (0.04)  & (0.04)  & (0.04)  & (0.04)  & (0.04)  \\  & [    0.06]  & [    0.16]  & [    0.24]  & [    0.11]  & [    0.09]  & [    0.24]  \\ \addlinespace[1ex] 
% \multicolumn{11}{l}{\emph{Panel B. Alternative hours thresholds}}  \\ 
% \addlinespace[1ex] \multirow[t]{ 3 }{0.2\textwidth}{Employed (0 hr) }  &      0.05 &      0.05 &      0.07 &      0.02 &      0.06 &      0.06 &      0.70 &      1770 &      0.12 &      0.46 \\ 
%  & (0.03)  & (0.04)  & (0.04)  & (0.04)  & (0.04)  & (0.04)  \\  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  \\ \addlinespace[1ex] 
% \multirow[t]{ 3 }{0.2\textwidth}{Employed (10 hr) }  &      0.02 &      0.03 &      0.05 &      0.00 &      0.01 &      0.01 &      0.48 &      1770 &      0.16 &      0.95 \\ 
%  & (0.03)  & (0.05)  & (0.05)  & (0.05)  & (0.05)  & (0.04)  \\  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  \\ \addlinespace[1ex] 
% \multirow[t]{ 3 }{0.2\textwidth}{Employed (20 hr) }  &      0.04 &      0.04 &      0.08 &      0.02 &      0.01 &      0.04 &      0.29 &      1770 &      0.17 &      0.62 \\ 
%  & (0.03)  & (0.04)  & (0.04)  & (0.04)  & (0.04)  & (0.04)  \\  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  \\ \addlinespace[1ex] 
% \multirow[t]{ 3 }{0.2\textwidth}{Employed (30 hr) }  &      0.02 &      0.03 &      0.09 &      0.04 &      0.00 &      0.06 &      0.19 &      1770 &      0.17 &      0.37 \\ 
%  & (0.03)  & (0.04)  & (0.04)  & (0.04)  & (0.04)  & (0.04)  \\  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  \\ \addlinespace[1ex] 
% \multirow[t]{ 3 }{0.2\textwidth}{Employed (40 hr) }  &      0.03 &      0.03 &      0.09 &     -0.01 &      0.02 &      0.04 &      0.13 &      1770 &      0.17 &      0.26 \\ 
%  & (0.02)  & (0.03)  & (0.04)  & (0.03)  & (0.03)  & (0.03)  \\  & [    1.00]  & [    1.00]  & [    0.70]  & [    1.00]  & [    1.00]  & [    1.00]  \\ \addlinespace[1ex] 
\bottomrule
\end{tabular}



==> tables/employment_breakdown_B.tex <==
\begin{tabular}{l *{6}{S} ScSS}
\toprule
 & & \multicolumn{4}{c}{GiveDirectly} & & \multicolumn{1}{c}{\raisebox{-1ex}[0pt]{Control}} \\ 
\cmidrule(lr){3-6}
\multicolumn{1}{c}{\text{ }} & \multicolumn{1}{c}{\text{HD}} & \multicolumn{1}{c}{\text{Lower}} & \multicolumn{1}{c}{\text{Middle}} & \multicolumn{1}{c}{\text{Upper}} & \multicolumn{1}{c}{\text{Large}} & \multicolumn{1}{c}{\text{Combined}} & \multicolumn{1}{c}{\text{Mean}} & \multicolumn{1}{c}{\text{Obs.}} & \multicolumn{1}{c}{\text{$ R^2$}} & \multicolumn{1}{c}{\text{$ p$-value}}\\
\midrule
% \multicolumn{11}{l}{\emph{Panel A. Employment composition}}  \\ 
% \addlinespace[1ex] \multirow[t]{ 3 }{0.2\textwidth}{Non-agricultural microenterprise }  &      0.05 &      0.09\ensuremath{^{*}} &      0.08\ensuremath{^{*}} &      0.14\ensuremath{^{**}} &      0.17\ensuremath{^{***}} &      0.12\ensuremath{^{**}} &      0.22 &      1770 &      0.12 &      0.00 \\ 
%  & (0.03)  & (0.04)  & (0.04)  & (0.05)  & (0.04)  & (0.04)  \\  & [    0.11]  & [    0.06]  & [    0.08]  & [    0.02]  & [    0.00]  & [    0.02]  \\ \addlinespace[1ex] 
% \multirow[t]{ 3 }{0.2\textwidth}{Other microenterprise or self-employment }  &      0.04\ensuremath{^{*}} &      0.04 &      0.11\ensuremath{^{**}} &      0.07\ensuremath{^{*}} &      0.05\ensuremath{^{*}} &      0.04 &      0.07 &      1770 &      0.09 &      0.02 \\ 
%  & (0.02)  & (0.03)  & (0.03)  & (0.03)  & (0.03)  & (0.03)  \\  & [    0.06]  & [    0.11]  & [    0.02]  & [    0.06]  & [    0.09]  & [    0.11]  \\ \addlinespace[1ex] 
% \multirow[t]{ 3 }{0.2\textwidth}{Agricultural processing or trading }  &      0.01 &      0.13\ensuremath{^{**}} &      0.01 &      0.07\ensuremath{^{*}} &      0.06 &      0.02 &      0.17 &      1770 &      0.08 &      0.05 \\ 
%  & (0.03)  & (0.04)  & (0.04)  & (0.04)  & (0.04)  & (0.04)  \\  & [    0.24]  & [    0.02]  & [    0.24]  & [    0.08]  & [    0.11]  & [    0.24]  \\ \addlinespace[1ex] 
% \multirow[t]{ 3 }{0.2\textwidth}{Agricultural wage labor }  &     -0.02 &     -0.08\ensuremath{^{**}} &     -0.07\ensuremath{^{*}} &     -0.08\ensuremath{^{**}} &     -0.11\ensuremath{^{**}} &     -0.09\ensuremath{^{**}} &      0.22 &      1770 &      0.15 &      0.00 \\ 
%  & (0.03)  & (0.03)  & (0.03)  & (0.03)  & (0.03)  & (0.03)  \\  & [    0.24]  & [    0.03]  & [    0.06]  & [    0.03]  & [    0.02]  & [    0.03]  \\ \addlinespace[1ex] 
% \multirow[t]{ 3 }{0.2\textwidth}{Non-agricultural wage labor }  &      0.06\ensuremath{^{*}} &     -0.04 &      0.01 &     -0.06 &     -0.07\ensuremath{^{*}} &      0.01 &      0.30 &      1770 &      0.20 &      0.00 \\ 
%  & (0.03)  & (0.04)  & (0.04)  & (0.04)  & (0.04)  & (0.04)  \\  & [    0.06]  & [    0.16]  & [    0.24]  & [    0.11]  & [    0.09]  & [    0.24]  \\ \addlinespace[1ex] 
\multicolumn{11}{l}{\emph{Panel B. Alternative hours thresholds}}  \\ 
\addlinespace[1ex] \multirow[t]{ 3 }{0.2\textwidth}{Employed (0 hr) }  &      0.05 &      0.05 &      0.07 &      0.02 &      0.06 &      0.06 &      0.70 &      1770 &      0.12 &      0.46 \\ 
 & (0.03)  & (0.04)  & (0.04)  & (0.04)  & (0.04)  & (0.04)  \\  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  \\ \addlinespace[1ex] 
\multirow[t]{ 3 }{0.2\textwidth}{Employed (10 hr) }  &      0.02 &      0.03 &      0.05 &      0.00 &      0.01 &      0.01 &      0.48 &      1770 &      0.16 &      0.95 \\ 
 & (0.03)  & (0.05)  & (0.05)  & (0.05)  & (0.05)  & (0.04)  \\  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  \\ \addlinespace[1ex] 
\multirow[t]{ 3 }{0.2\textwidth}{Employed (20 hr) }  &      0.04 &      0.04 &      0.08 &      0.02 &      0.01 &      0.04 &      0.29 &      1770 &      0.17 &      0.62 \\ 
 & (0.03)  & (0.04)  & (0.04)  & (0.04)  & (0.04)  & (0.04)  \\  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  \\ \addlinespace[1ex] 
\multirow[t]{ 3 }{0.2\textwidth}{Employed (30 hr) }  &      0.02 &      0.03 &      0.09 &      0.04 &      0.00 &      0.06 &      0.19 &      1770 &      0.17 &      0.37 \\ 
 & (0.03)  & (0.04)  & (0.04)  & (0.04)  & (0.04)  & (0.04)  \\  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  & [    1.00]  \\ \addlinespace[1ex] 
\multirow[t]{ 3 }{0.2\textwidth}{Employed (40 hr) }  &      0.03 &      0.03 &      0.09 &     -0.01 &      0.02 &      0.04 &      0.13 &      1770 &      0.17 &      0.26 \\ 
 & (0.02)  & (0.03)  & (0.04)  & (0.03)  & (0.03)  & (0.03)  \\  & [    1.00]  & [    1.00]  & [    0.70]  & [    1.00]  & [    1.00]  & [    1.00]  \\ \addlinespace[1ex] 
\bottomrule
\end{tabular}


